Identity-Based Authentication for On-Demand Charging of Electric Vehicles

Dynamic wireless power transfer provides means for charging Electric Vehicles (EVs) while driving, avoiding stopping for charging and hence fostering their widespread adoption. Researchers devoted much effort over the last decade to provide a reliable infrastructure for potential users to improve comfort and time management. Due to the severe security and performance system requirements, the different scheme proposed in last years lack of a unified protocol involving the modern architecture model with merged authentication and billing processes. Furthermore, they require the continuous interaction of the trusted entity during the process, increasing the delay for the communication and reducing security due to the large number of message exchanges. In this paper, we propose a secure, computationally lightweight, unified protocol for fast authentication and billing that provides on-demand dynamic charging to comprehensively deal with all the computational and security constraints. The protocol employs an ID-based public encryption scheme to manage mutual authentication and pseudonyms to preserve the user's identity across multiple charging processes. Compared to state-of-the-art authentication protocols, our proposal overcomes the problem of overwhelming interactions and provides public scheme security against the use of simple operations in wide open communications without impacting on performance.

==> sections/7_4_informal_analysis.tex <==
\section{Informal Security Analysis}

In this section we assess that the protocol provides the services required and that it is secure against well-known attacks with an informal security analysis. 
% requirements
The system requires to provide:
\begin{itemize}
    \item Mutual authentication: the protocol requires mutual authentication between the CSPA and EV that wants to receive the charge. The ID-based public-key cryptography grants this on the bilinear map, where only registered entities can derive mutual secrets without errors.
    \item Privacy-preserving: the proposed scheme hides the customers' real identity using pseudonyms generated from a random seed and updated with a non-linear function. The EV does not share its real identity with the charging infrastructure during the entire authentication protocol.
    % \item Integrity: ???? we don't have hash checking (tag appending solution)
    \item Bidirectional auditability and  Non-repudiation: EV and CSPA compute the total amount of pads used in the charging process. The user, after the billing, can dispute the amount charged by the CSPA in case she/he finds it different. The tamper-proof OBU guarantees the possibility to verify if this is the case.
    \item Perfect Forward Secrecy: thanks to the assumptions in the Diffie-Hellman problem, the perfect forward secrecy is guaranteed. If a key is compromised, the previous messages are still secure from an adversary who wants to know the content. 
\end{itemize}

% attacks and protection
The protocol is proven to be secure against the most common attacks in this scenario:
\begin{itemize}
    \item Unlinkability: every pseudonym is generated from a secret seed and an initial parameter stored in the OBU (Tamper-Proof) and the RA server. The generation follows the rule previously stated as the concatenation of the real identity of the EV and a (non-linear) function of the seed and parameter, then hashed with a cryptographic hash function (pre-image and collision-resistant). In this way, it is impossible to predict the pseudonym generated without knowing the initial parameters, and it is impossible to correlate them.
    \item Man-In-The-Middle: in this scenario, the adversary stands in between the conversation of two legitimate parties. This attack is not a risk because the adversary cannot gain anything by standing between either party communicating. This is due to implementing the message authentication code in bilinear mapping based on a secret given by RA to EV, which is the key for the pseudonym. The adversary cannot forward the resulting \textit{mac} to the CSPA during the communication and get a valid authentication at the CSPA side.
    %\item Known key: ?
    %\item Denial-of-Service: don't think it is resistant: a malicious user could send tons of m3s and CSPA would generate nonces and randoms indefinitely. Even the other papers I don't think they are really safe.
    \item Free-riding: in this situation, a malicious user attempts to get a free charge without being authenticated. The attack is mitigated as the hash chain used for authenticating with the CP can be generated only by the intended user. The adversary could listen to the current value to authenticate with the next pad. However, the successive charging plate will wait for the next value of the has chain to authenticate the EV. This value cannot be computed by an unauthenticated, different vehicle.
    \item Double-spending: in this scenario, an EV that just utilized the service wants to use the same message again to get a free charge. This can be avoided by using timestamps and the token validity time, the time after which the EV cannot use the same token for another charge.
\end{itemize}



==> sections/params_size_table.tex <==
\begin{table}[h!]
\begin{center}
    \begin{tabular}{| p{2.5cm} | p{2.5cm} |}
        \hline
        \textbf{Parameter} & \textbf{Size (Bytes)}\\
        \hline
        $ID$ & 32  \\
        \hline
        $PID$ & 32  \\
        \hline
        $N$ & 32  \\
        \hline
        $r$ & 32  \\
        \hline
        $P$ & 32  \\
        \hline
        $t$ & 8  \\
        \hline
        $ticket$ & 64  \\
        \hline
        $mac$ & 32  \\
        \hline
        $T$ & 32  \\
        \hline
        $h(T)$ & 32  \\
        \hline
        $sk$ &  32 \\
        \hline
    \end{tabular}
    \caption{Parameter costs in bytes}
    \label{table:communication_sizes}
\end{center}
\end{table}


==> sections/seq_diagram.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=18cm, height = 9cm]{images/protocol_diagram.png}
    \caption{Sequence diagram of the authentication protocol}
    \label{fig:seq_diagram}
\end{figure*}

